Sponge: Inference Serving with Dynamic SLOs Using In-Place Vertical Scaling

Mobile and IoT applications increasingly adopt deep learning inference to provide intelligence. Inference requests are typically sent to a cloud infrastructure over a wireless network that is highly variable, leading to the challenge of dynamic Service Level Objectives (SLOs) at the request level. This paper presents Sponge, a novel deep learning inference serving system that maximizes resource efficiency while guaranteeing dynamic SLOs. Sponge achieves its goal by applying in-place vertical scaling, dynamic batching, and request reordering. Specifically, we introduce an Integer Programming formulation to capture the resource allocation problem, providing a mathematical model of the relationship between latency, batch size, and resources. We demonstrate the potential of Sponge through a prototype implementation and preliminary experiments and discuss future works.

==> old_tex_files/03-problem.tex <==
\section{Problem Formulation} \label{sec:architecture}
\subsection{Reconciling Vertical Scaling and Batch size}
FIGURE + FORMULATION
\subsection{IP}



\subsection{Solution}


\iffalse
where:
\begin{itemize}
    \item $R$ represents the set of all requests.
    \item $S$ represents the set of all components.
    \item $R_s$ is the set of requests that use service.
    % \item $|R_s|$ is the number of requests associated with service.
    \item $n_s$ is the number of instances per component of service $s$.
    \item $V_s$ represents the set of variants for component $s$.
    \item $x_{s,v}$ is a binary decision variable representing whether variant $v$ of component $s$ is chosen.
    \item $cc_r$ is the communication cost associated with request $r$.
    \item $SLA_r$ is the SLA requirement for request $r$.
    \item $d_{s,v}(b_s)$ is the processing time of service $s$ with variant $v$ and batch size $b_s$.
    \item $q_s(b_s)$ is the queuing time of service $s$ and batch size $b_s$.
    \item $d_{s,v}(b_s)$ is the throughput  of service $s$ with variant $v$ and batch size $b_s$.
\end{itemize}

\begin{equation}
    \begin{aligned}
        \text{Minimize} \quad & \sum_{s \in S} n_s \\
        \text{subject to} \quad & \sum_{r \in R} d_{s,v}(b_s) + q_{s,v}(b_s) + \text{cc}_r \leq \text{SLA}_r, \quad \forall r \in R \\
        & h_{s,v}(b_s) \cdot n_s \geq \sum_{r \in R_s} \lambda_r, \quad \forall s \in S\\
        & \text{Accuracy}_s \geq \alpha, \quad \forall s \in S\\
        & b_s, n_s \in \mathbb{Z}^+, \quad \forall s \in S \\
        & x_{s,v} \in \{0, 1\}, \quad \forall s \in S, v \in V_s \\
        & \sum_{v \in V_s} x_{s,v} = 1, \quad \forall s \in S \\
    \end{aligned}
\end{equation}

where:
\begin{itemize}
    \item $R$ represents the set of all requests.
    \item $S$ represents the set of all components.
    \item $R_s$ is the set of requests that use service.
    % \item $|R_s|$ is the number of requests associated with service.
    \item $n_s$ is the number of instances per component of service $s$.
    \item $Accuracy_{s,v}$ is the accuracy for service $s$ with variant $v$.
    \item $\alpha$ is the minimum accuracy threshold.
    \item $V_s$ represents the set of variants for component $s$.
    \item $x_{s,v}$ is a binary decision variable representing whether variant $v$ of component $s$ is chosen.
    \item $cc_r$ is the communication cost associated with request $r$.
    \item $SLA_r$ is the SLA requirement for request $r$.
    \item $d_{s,v}(b_s)$ is the processing time of service $s$ with variant $v$ and batch size $b_s$.
    \item $q_s(b_s)$ is the queuing time of service $s$ and batch size $b_s$.
    \item $d_{s,v}(b_s)$ is the throughput  of service $s$ with variant $v$ and batch size $b_s$.
\end{itemize}
\fi

==> old_tex_files/05-implementation.tex <==
\section{Implementation} \label{sec:implementation}


==> old_tex_files/10-extra.tex <==
\section{Extra}


